Cross-Stack Workload Characterization of Deep Recommendation Systems

Deep learning based recommendation systems form the backbone of most personalized cloud services. Though the computer architecture community has recently started to take notice of deep recommendation inference, the resulting solutions have taken wildly different approaches - ranging from near memory processing to at-scale optimizations. To better design future hardware systems for deep recommendation inference, we must first systematically examine and characterize the underlying systems-level impact of design decisions across the different levels of the execution stack. In this paper, we characterize eight industry-representative deep recommendation models at three different levels of the execution stack: algorithms and software, systems platforms, and hardware microarchitectures. Through this cross-stack characterization, we first show that system deployment choices (i.e., CPUs or GPUs, batch size granularity) can give us up to 15x speedup. To better understand the bottlenecks for further optimization, we look at both software operator usage breakdown and CPU frontend and backend microarchitectural inefficiencies. Finally, we model the correlation between key algorithmic model architecture features and hardware bottlenecks, revealing the absence of a single dominant algorithmic component behind each hardware bottleneck.

==> tables/hw_wide.tex <==
\begin{table*}[t]
\begin{center}
\resizebox{\linewidth}{!}{\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Machines}                    & \textbf{Xeon E5-2697A v4} & \textbf{Xeon Gold 6242} & \textbf{GTX 1080 Ti} & \textbf{T4} \\ \hline
Microarchitecture                    & Broadwell                 & Cascade Lake            & Pascal               & Turing      \\ \hline
Frequency                            & 2.6 GHz                   & 2.8 GHz                 & 1.48 GHz             & 0.58 GHz    \\ \hline
Cores per socket (SM Count)          & 16                        & 16                      & (28)                 & (40)        \\ \hline
Sockets                              & 2                         & 2                       & N/A                  & N/A         \\ \hline
SIMD (CUDA Compute Capability)       & AVX-2                     & AVX-512                 & (6.1)                & (7.5)       \\ \hline
L1 Cache Size                        & 32 KB                     & 32 KB                   & 48 KB                & 64 KB       \\ \hline
L2 Cache Size                        & 256 KB                    & 1 MB                    & 2.75 MB              & 4 MB        \\ \hline
L3 Cache Size                        & 40 MB                     & 22 MB                   & N/A                  & N/A         \\ \hline
L2/L3 (L1/L2) Cache Inclusion Policy & Inclusive                 & Exclusive               & Inclusive            & Inclusive   \\ \hline
DRAM Capacity                        & 256 GB                    & 384 GB                  & 11 GB                & 16 GB       \\ \hline
DDR Type                             & DDR4                      & DDR4                    & GDDR5X               & GDDR6       \\ \hline
DDR Frequency                        & 2400 MHz                  & 2933 MHz                & 1376 MHz             & 1250 MHz    \\ \hline
DDR Bandwidth per socket             & 77 GB/s                   & 131 GB/s                & 484.4 GB/s           & 320 GB/s    \\ \hline
TDP                                  & 145 W                     & 150 W                   & 250 W                & 70 W        \\ \hline
\end{tabular}}
\end{center}
\caption{Summary of Hardware Platforms}
\label{tab:hw}
\end{table*}

==> tables/rec_models.tex <==
\begin{table}[t]
\begin{center}
\resizebox{\linewidth}{!}{\begin{tabular}{|c||c|c|}
\hline
\textbf{Model} & \textbf{Application Domain (Evaluation Case)} & \textbf{Algorithmic Insight}                                                                                                                                  \\ \hline
NCF            & Movies (MovieLens)                            & Small model with only four embedding tables                                                                                                                   \\ \hline
RM1            & Social Media (Facebook)                       & \begin{tabular}[c]{@{}c@{}}Small model with medium amount ($\sim80$) \\ of lookups per embedding table\end{tabular}                                                 \\ \hline
RM2            & Social Media (Facebook)                       & \begin{tabular}[c]{@{}c@{}}Large model with large amount ($\sim120$) \\ of lookups per embedding table\end{tabular}                                                 \\ \hline
RM3            & Social Media (Facebook)                       & \begin{tabular}[c]{@{}c@{}}Large model with large FC stacks \\ and immediate continuous input processing\end{tabular}                                         \\ \hline
WnD            & Smartphone Apps (Google Play Store)           & Medium model with large FC stacks                                                                                                                             \\ \hline
MT-WnD         & Video (YouTube)                               & \begin{tabular}[c]{@{}c@{}}Large model with multiple parallel FC stacks\\  on top of WnD\end{tabular}                                                         \\ \hline
DIN            & E-Commerce (Alibaba)                          & \begin{tabular}[c]{@{}c@{}}Large model with local activation weights \\ for large amount ($\sim750$) of lookups \\ from user behavior embedding tables\end{tabular} \\ \hline
DIEN           & E-Commerce (Alibaba - Taobao)                 & \begin{tabular}[c]{@{}c@{}}Medium model with interaction GRUs to replace \\ large amount of lookups found in DIN\end{tabular}                                 \\ \hline
\end{tabular}}
\end{center}
\caption{Summary of Recommendation Models}
\label{tab:rec_models}
\end{table}
